Back to the Future: Unsupervised Backprop-based Decoding for Counterfactual and Abductive Commonsense Reasoning

Abductive and counterfactual reasoning, core abilities of everyday human cognition, require reasoning about what might have happened at time t, while conditioning on multiple contexts from the relative past and future. However, simultaneous incorporation of past and future contexts using generative language models (LMs) can be challenging, as they are trained either to condition only on the past context or to perform narrowly scoped text-infilling. In this paper, we propose DeLorean, a new unsupervised decoding algorithm that can flexibly incorporate both the past and future contexts using only off-the-shelf, left-to-right language models and no supervision. The key intuition of our algorithm is incorporating the future through back-propagation, during which, we only update the internal representation of the output while fixing the model parameters. By alternating between forward and backward propagation, DeLorean can decode the output representation that reflects both the left and right contexts. We demonstrate that our approach is general and applicable to two nonmonotonic reasoning tasks: abductive text generation and counterfactual story revision, where DeLorean outperforms a range of unsupervised and some supervised methods, based on automatic and human evaluation.

==> 4-task.tex <==
\section{Tasks}
\label{sec:task}

\vered{since we already described the tasks previously, we might need a different title for this section, something like ``task-specific setup''.}

\vered{Instead of splitting each section to two subsection, one for each task, consider having one ``counterfactual reasoning'' section with the setup, results, baselines, etc. and another section for abductive reasoning.}

\subsection{Counterfactual Reasoning}
\label{ssec:tasks:counterfactual}

We are given an original story ending $Y^{ori}=(y^{ori}_1,\dots,y^{ori}_N)$ of an original context $X^{ori}$. We are further given a new context $X$ which is counterfactual to $X^{ori}$. The task is to generate a new story ending $Y$ that is consistent with $X$ and at the same time minimally edits the original ending $Y^{ori}$~\cite{qin2019counterfactual}.

Therefore, the constraint here is that $Y$ needs to be close to $Y^{ori}$. Using our proposed framework, a straightforward way of imposing the constraint is to minimize their KL divergence:
\begin{equation}
\begin{split}
\mathcal{L}(\Tilde{Y}) :=& \text{KL}\left( Y^{ori} \| \text{softmax}(\Tilde{Y}/\tau) \right),  
\end{split}
\end{equation}
where, with a slight abuse of notations, $Y^{ori}$ is the one-hot distribution of the tokens in the original ending. That is, we encourage the generated logits to recover the original ending.

\paragraph{Ranking}
We rank the candidates based on both their coherence with the context, as well as the internal coherence between the multiple sentences of each candidate. More concretely, given a candidate $Y$, we compute the aggregated coherence score:
\begin{equation}
\begin{split}
&\operatorname{ranking\_score}(Y) = \\ 
&c(X, Y) + \sum_{s=1}^{S-1} c(Y[s], Y[s+1]),
\end{split}
\end{equation}
where each candidate has $S$ sentences and $Y[s]$ denotes the $s$th sentence.


\subsection{Abductive Reasoning}
\label{ssec:tasks:abductive}

We are given a premise $X$ as well as an ending $Z$. The task is to generate an explanation $Y$ such that $(X,Y,Z)$ forms a coherent story. In other words, $Y$ must take into account both the left-side context $X$ and the right-side context $Z$.

To this end, we define the loss function as the cross-entropy loss of generating $Z$ given $Y$ based on the LM:
\begin{equation}
\begin{split}
\mathcal{L}(\Tilde{Y}) :=& - \log P_{\LM}(Z|X,\Tilde{Y}) \\
=& - \sum_{n=1}^{N_{Z}} \log P_{\LM}(z_n | X,\Tilde{Y}, Z_{1:n-1}),
\end{split}
\end{equation}
where $P_{\LM}(z_n | X, \Tilde{Y}, Z_{1:n-1})$ is the likelihood of generating token $z_n$ by the LM given the preceding text $(X, \Tilde{Y}, Z_{1:n-1})$.

\paragraph{Ranking}
Based on the problem definition, we rank candidates according to the consistency after inserting $Y$ in between $X$ and $Z$:
\begin{equation}
% \begin{split}
\resizebox{0.89\hsize}{!}{%
$\operatorname{ranking\_score}(Y) = c(XY, Z) + c(X, YZ).$%
}
% \end{split}
\end{equation}
That is, we concatenate $X$ and $Y$ as a single piece of text and evaluate its consistency with the subsequent $Z$, and similarly, we concatenate $Y$ and $Z$ and evaluate the consistency between $X$ and $YZ$.

% \begin{equation}
% \begin{split}
% \mathcal{L}(\Tilde{Y}) :=& - 2 \log P_{\LM}(Z|\Tilde{Y}, X) \\
% & + \log P_{\LM}(Z|\Tilde{Y}) \\
% & + \log P_{\LM}(Z|X)
% \end{split}
% \end{equation}

==> 5-setup.tex <==
\section{Experimental Setup}
\label{sec:setup}

\subsection{Counterfactual Reasoning}
\label{ssec:setup:counterfactual}

\paragraph{Hyperparameters}

\paragraph{Baselines} As baselines, we report the performance of models from \citet{qin2019counterfactual}. These models are fine-tuned from \textbf{GPT2-345M} \citet{radford2019language} and trained on additional domain-relevant datasets with varying training objectives. The \texttt{ZS} model generates counterfactual alternatives solely from the pretrained \textbf{GPT2-345M} model. The \texttt{FT} model fine-tunes \textbf{GPT2-345M} on in-domain data from the \textsc{RocStories} corpus \cite{mostafazadeh2016corpus}. Similarly, the \texttt{FT + CF} model is an extension of the \texttt{FT} model that also includes fine-tuning on the counterfactual prompts from the dataset of \citet{qin2019counterfactual}. In contrast to these generative adaptation losses, the \texttt{Recon} model is discriminative, conditioning on original stories and using an autoencoding objective to encourage the same ending to be produce given the counterfactual alternative. Finally, the \texttt{Sup} model uses the counterfactual training set endings of \citet{qin2019counterfactual} to train a supervised model for counterfactual generation.


% \begin{itemize}
%     \item unsupervised models from \citet{qin2019counterfactual}
%     \item supervised models from \citet{qin2019counterfactual}
%     \item zero-shot models from \citet{qin2019counterfactual}
% \end{itemize}

\paragraph{Ablations}

\paragraph{Metrics} We report the automatic metrics from \cite{qin2019counterfactual} that are most closely correlated with human judgments: ROUGE-L \cite{lin2004rouge} and \textsc{BertScore} \cite{Zhang2019BERTScoreET}. We also report the results of a human evaluation along the following dimensions: \antoine{fill this in}

% \begin{itemize}
%     \item Same as from \citet{qin2019counterfactual}
% \end{itemize}

\subsection{Abductive Reasoning}
\label{ssec:setup:abductive}

\paragraph{Hyperparameters}

\paragraph{Baselines} We report baseline models first proposed in \citet{bhagavatula2019abductive}. The \texttt{GPT2-Fixed} model concatenates $X$ and $Y$ followed by a ``because" token as a means of inducing a justification for $Y$. The $X$-$Y$\texttt{-only} model is fine-tuned on the ART dataset to generate the correct hypothesis given both $X$ and $Y$ as input. Finally, the \texttt{COMeT-Emb+GPT2} model is an augmentation of $X$-$Y$\texttt{-only} that prepends commonsense representation vectors to the beginning of the input sequence. These vectors are produced by a neural knowledge base, \textsc{COMET} \cite{bosselut-etal-2019-comet}, trained on the \textsc{Atomic} knowledge graph \cite{Sap2019ATOMICAA}. Both $X$ and $Y$ are input to \textsc{COMET} and a vector is produce for each commonsense dimension from \textsc{Atomic} learned by \textsc{COMET}. 
While these models originally use \textbf{GPT2-117M} \cite{radford2019language} as a pretrained starting point, we update their initialization to \textbf{GPT2-345M} to be in line with our own approach. 
\begin{itemize}
    \item Supervised models from \citet{bhagavatula2019abductive}
    \item Supervised; $P(\Tilde{Y} | O_1)$
    \item Zero-shot; $P(\Tilde{Y} | O_1)$
    \item Zero-shot $P(\Tilde{Y} | O_1)$, re-rank using $P(O_2 | \Tilde{Y})$
    \item Zero-shot $P(\Tilde{Y} | O_1)$, re-rank using $P(O_2 | \Tilde{Y}, O_1)$
\end{itemize}

\paragraph{Ablations}

\paragraph{Metrics}

\begin{itemize}
    \item Same as from \citet{bhagavatula2019abductive}
\end{itemize}

==> 6-experiments.tex <==
\section{Experiments}
\label{sec:experiments}

%%%%%%% Counterfactual %%%%%%%%%%%

\input{emnlp2020-templates/figure/counterfactual_human_calibration}
\input{emnlp2020-templates/figure/counterfactual_human_pairwise}
\input{emnlp2020-templates/figure/counterfactual_automatic}


%%%%%%% Abductive %%%%%%%%%%%

\input{emnlp2020-templates/figure/abductive_human_calibration}
\input{emnlp2020-templates/figure/abductive_human_pairwise}
\input{emnlp2020-templates/figure/abductive_automatic}



==> abstract.tex <==
Abductive and counterfactual reasoning, core abilities of everyday human cognition, require reasoning about what might have happened at time t, while conditioning on multiple contexts from the relative past and future. However, simultaneous incorporation of past and future contexts using generative language models (LMs) can be challenging, as they are trained either to condition only on the past context or to perform narrowly scoped text-infilling. 

In this paper, we propose DeLorean, a new unsupervised decoding algorithm that can flexibly incorporate both the past and future contexts using only off-the-shelf, left-to-right language models and no supervision. The key intuition of our algorithm is incorporating the future through back-propagation, during which, we only update the internal representation of the output while fixing the model parameters. By alternating between forward and backward propagation, DeLorean can decode the output representation that reflects both the left and right contexts. We demonstrate that our approach is general and applicable to two nonmonotonic reasoning tasks: abductive text  generation and counterfactual story revision, where DeLorean outperforms a range of unsupervised and some supervised methods, based on automatic and human evaluation.

==> emnlp2020-templates/figure/abductive_sampling_table.tex <==
% \usepackage{colortbl}

% {ccc} 
\begin{table*}
\centering
\scalebox{0.9}{
\begin{tabular}{lcl}
\cmidrule[\heavyrulewidth]{1-3}
\rowcolor[gray]{0.95} \textbf{Observation 1 (Input)} & \textbf{Hypothesis (Output)}      & \textbf{Observation 2 (Input)}  \\
% \rowcolor[rgb]{0.898,0.898,0.898} \textbf{t} & \multicolumn{1}{c}{\textbf{Generated Y}}      & \textbf{Score}  \\
In April, Bob decided he need to do his taxes.  & Bob then went to the IRS to do his.  & The accountant prepared and filed Bob's taxes. \\
Ray drive his car on a steep mountain road.  & As he drives the car to the top of the mountain his car is hit by a car. & Ray was fine but his car was totaled.                     \\
Ed likes to buy vintage records. &  He says he's always been a collector, and they're a great way to get into the music business. &He won't say what they cost him, though.                      \\
\cmidrule[\heavyrulewidth]{1-3}
\end{tabular}
}
\vspace{-5pt}
\caption{A sample of generated abductive reasoning hypotheses and their ranking scores.}
\label{tab:abd_sample}
\end{table*}

==> emnlp2020-templates/figure/counterfactual_sampling_table.tex <==
% \usepackage{caption}
% \usepackage{booktabs}
% \usepackage{colortbl}


\begin{table*}
\centering
\small
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
% \captionsetup{labelformat=empty}
\scalebox{0.85}{
\begin{tabular}{lll} 
\toprule
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{Story Beginning (${X}^{Ori}$: $s1,s2$):~~}I wanted a pet for my birthday.~I wasn't sure what to get, I already had dogs.\\
\textbf{Counterfactual (${X}$: $s1,s2^'$):~ }I wanted a pet for my birthday.~Only dogs are allowed in my apartment building.\\
\textbf{Story Ending (${Z}$: $s3,s4,s5$):~ }I was looking around on facebook and saw a mini pig. I went to pick her up. I drove home with the mini pig.\\\end{tabular}}  \\ 
\midrule
\rowcolor[rgb]{0.898,0.898,0.898} \textbf{t} & \multicolumn{1}{c}{\textbf{Generated Y: $s3^'$, $s4^'$, $s5^'$}}      & \textbf{Score}  \\
1                                    & I was looking for a dog and I found this one. I was so happy to find a dog that I could take care of. I love him and he is so sweet.                                 & 4.04                                                                                                                                                                                      \\
2                                    & I was looking for a dog and I found this one. I went to the vet and he said it was a good dog. I was so happy.                                                       & 4.02                                                                                                                                                                                      \\
3                                    & I was looking around on facebook and saw a dog. I went to the pet store and bought the dog. I was so excited to get my dog.                                          & \textbf{5.08}                                                                                                                                                                                      \\
4                                    & I was looking around on the internet for a pet and I found this website. I went to pick her up. I was so excited to see her.                                         & 2.75                                                                                                                                                                                      \\
5                                    & I was looking around on the internet for a pet. I found a dog named "Bubba". I was so excited to have a dog. & 5.07                                                                                                                                                                                      \\
\bottomrule
\end{tabular}
}
\caption{Samples of \modelname{}-generated texts for the counterfactual reasoning task.}
\label{tab:counter_sample}
\end{table*}
